Enhancing Recipe Retrieval with Foundation Models: A Data Augmentation Perspective

Learning recipe and food image representation in common embedding space is non-trivial but crucial for cross-modal recipe retrieval. In this paper, we propose a new perspective for this problem by utilizing foundation models for data augmentation. Leveraging on the remarkable capabilities of foundation models (i.e., Llama2 and SAM), we propose to augment recipe and food image by extracting alignable information related to the counterpart. Specifically, Llama2 is employed to generate a textual description from the recipe, aiming to capture the visual cues of a food image, and SAM is used to produce image segments that correspond to key ingredients in the recipe. To make full use of the augmented data, we introduce Data Augmented Retrieval framework (DAR) to enhance recipe and image representation learning for cross-modal retrieval. We first inject adapter layers to pre-trained CLIP model to reduce computation cost rather than fully fine-tuning all the parameters. In addition, multi-level circle loss is proposed to align the original and augmented data pairs, which assigns different penalties for positive and negative pairs. On the Recipe1M dataset, our DAR outperforms all existing methods by a large margin. Extensive ablation studies validate the effectiveness of each component of DAR.

==> figs/segment_handmade.tex <==
% Use figure* for multi-column figure
\begin{figure}[]
    \centering
    %%\includegraphics[width=\linewidth]{figs/overview.png}
    \includegraphics[width=0.9\linewidth]{figs/segments_handmade_true.pdf}
    % \captionsetup{justification=centering}
    \caption{ Qualitative examples qualitative example of the effect of SAM imperfections on retrieval. The first three columns are the image query, the segments automatically generated by SAM, and the segments selected interactively with SAM manually. The DAR++'s Top-5  retrieved recipes with hand-selected segments are represented by word clouds. The blue
boxes represent the ground truth. The red boxes and purple boxes represent the Top-1 retrieved image of DAR and DAR++ with automatically generated segments, respectively.}
    \label{fig:segment_hand}
\end{figure}





==> figs/sim.tex <==
\begin{figure}[h]
    %\centering
    %%\includegraphics[width=\linewidth]{figs/overview.png}
    \includegraphics[width=\linewidth]{figs/similarity_test_visualization.pdf}
    %%\captionsetup{justification=centering}
    \caption{similarity matrix,From left to right, (a) the similarity matrix of the original image and the recipe, (b) the similarity matrix of the image and the visual imagnation, (c) the similarity matrix of the segment and the recipe, and (d) the result of multiplying the first three matrices together }
    \label{fig:sim}
\end{figure}

==> tables/ablation_augmentation_before.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Ablation study for augmented data. The operations are all added to the Baseline model.}

\resizebox{\textwidth}{!}{
\begin{tabular}{@{}clcccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Operation}}}                      & \multicolumn{4}{c}{\textbf{image-to-recipe}}                & \multicolumn{4}{c}{\textbf{recipe-to-image}}                \\ \cmidrule(l){3-10} 
                                & \multicolumn{1}{c}{}                                                         & \textbf{medR} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} & \textbf{medR} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} \\ \midrule
\textbf{Baseline}               & \multicolumn{1}{c}{}                                                         & 2.0           & 42.3         & 71.8         & 81.5          & 2.0           & 43.4         & 72.8         & 82.3          \\ \midrule
                                & + segments (\phi_{\text{seg}})                                        & 2.0           & 43.0         & 72.3         & 81.9          & 2.0           & 43.6         & 73.0         & 82.6          \\
                                & + description (\phi_{\text{dec\&A}})                                  & 2.0           & 43.7         & 72.6         & 82.0          & 2.0           & 44.7         & 73.9         & 83.1          \\ \midrule
\textbf{CAR}                    & + segment($\phi_{\text{seg}}$), description(\phi_{\text{dec\&A}}) & 2.0           & 44.2         & 73.2         & 82.4          & 2.0           & 44.8         & 73.9         & 83.1          \\ \bottomrule
\end{tabular}
}

\label{tab:ablation_augmentation1}
\end{table}

==> tables/ablation_llmprompt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{ Performance comparison of different prompt schemes for LLM based on the CAR model setup.}

\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Prompt}} & \multicolumn{4}{c}{\textbf{image-to-recipe}}                & \multicolumn{4}{c}{\textbf{recipe-to-image}}                \\ \cmidrule(l){2-9} 
                                 & \textbf{medR} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} & \textbf{medR} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} \\ \midrule
\textbf{Recipe Summary}          & 2.0           & 43.9         & 73.2         & 82.4          & 2.0           & 44.4         & 74.0         & 83.1          \\ \midrule
\textbf{Visual Imagination}      & 2.0           & 44.2         & 73.2         & 82.4          & 2.0           & 44.8        & 73.9         & 83.1          \\ \bottomrule
\end{tabular}


\label{tab:ablation_llmprompt}
\end{table}
